Dynamic Prompt Learning via Policy Gradient for Semi-structured Mathematical Reasoning

Mathematical reasoning, a core ability of human intelligence, presents unique challenges for machines in abstract thinking and logical reasoning. Recent large pre-trained language models such as GPT-3 have achieved remarkable progress on mathematical reasoning tasks written in text form, such as math word problems (MWP). However, it is unknown if the models can handle more complex problems that involve math reasoning over heterogeneous information, such as tabular data. To fill the gap, we present Tabular Math Word Problems (TabMWP), a new dataset containing 38,431 open-domain grade-level problems that require mathematical reasoning on both textual and tabular data. Each question in TabMWP is aligned with a tabular context, which is presented as an image, semi-structured text, and a structured table. There are two types of questions: free-text and multi-choice, and each problem is annotated with gold solutions to reveal the multi-step reasoning process. We evaluate different pre-trained models on TabMWP, including the GPT-3 model in a few-shot setting. As earlier studies suggest, since few-shot GPT-3 relies on the selection of in-context examples, its performance is unstable and can degrade to near chance. The unstable issue is more severe when handling complex problems like TabMWP. To mitigate this, we further propose a novel approach, PromptPG, which utilizes policy gradient to learn to select in-context examples from a small amount of training data and then constructs the corresponding prompt for the test example. Experimental results show that our method outperforms the best baseline by 5.31% on the accuracy metric and reduces the prediction variance significantly compared to random selection, which verifies its effectiveness in selecting in-context examples.

==> codes/results.tex <==
\begin{figure}[htb] 
 \centering
 \renewcommand\tabcolsep{4.0pt} % column space
%  \renewcommand\arraystretch{0.85} % row space
 \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{lcccccccccccc} 
    \toprule
    \multirow{3}{*}{Method} & \multirow{3}{*}{Learning} & \multirow{3}{*}{Format} & \multicolumn{2}{c}{Question Types} & \multicolumn{5}{c}{Answer Types} &
    \multicolumn{2}{c}{Grades} &
    \multirow{3}{*}{Avg} \\
    \cmidrule(lr){4-5} \cmidrule(lr){6-10} \cmidrule(lr){11-12} 
    & & & MC & Free-text & INT & DEC & EXTR & BOOL & OTH & 1-6 & 7-8 & \\
    \midrule
    Random guess & - & TQ(C)$\rightarrow$A & 38.15 & 7.13 & 9.78 & 0.43 & 29.79 & 48.44 & 28.57 & 16.80 & 13.00 & 15.17 \\
    Human performance & - & TQ(C)$\rightarrow$A & & & \\
    \midrule
    VisualBert & fine-tuning & TQ(C)$\rightarrow$A & & & \\
    ViLT & fine-tuning & TQ(C)$\rightarrow$A & & & \\
    \midrule
    TAPAS & zero-shot & TQ(C)$\rightarrow$A & & & \\
    TAPEX & zero-shot & TQ(C)$\rightarrow$A & & & \\
    \midrule    
    GPT-3  & zero-shot & TQ(C)$\rightarrow$A & 65.62 & 51.48 & 52.32 & 49.27 & 81.15 & 52.85 & 36.36 & 63.56 & 43.47 & 55.10 \\
    GPT-3 Step-by-step \citeyearpar{kojima2022large} & zero-shot & TQ(C)$\rightarrow$A & 67.97 & 55.11 & 55.54 & 53.38 & 80.33 & 57.72 & 45.45 & 63.73 & 51.07 & 58.40 \\
    GPT-3  & 2-shot & TQ(C)$\rightarrow$A & 65.23 & 54.84 & 56.40 & 50.73 & 79.51 & 52.85 & 45.45 & 64.77 & 47.51 & 57.50 \\
    GPT-3 CoT & 2-shot & TQ(C)$\rightarrow$SA & 58.20 & 58.60 & 55.47 & 66.83 & 64.75 & 52.85 & 45.45 & 62.69 & 52.73 & 58.50 \\
    
    Codex & 2-shot & TQ(C)$\rightarrow$A & & & & \\
    \midrule   
    GPT-3 RLPrompt (ours) & N-shot & TQ(C)$\rightarrow$SA & & & \\
    \bottomrule 
    \end{tabular}
 }
 \captionof{table}{Evaluation results of different baselines and our methods on the \data{} dataset. MC: multi-choice questions; Free-text: free-text questions; INT: integer answers; DEC: decimal answers; EXTR: extractive text answers; BOOL: boolean text answers; OTH: other text answers.}
 \label{tab:results1}
\end{figure}

\begin{figure}[htb] 
 \centering
 \renewcommand\tabcolsep{4.0pt} % column space
%  \renewcommand\arraystretch{0.85} % row space
 \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{lcccccccccccc} 
    \toprule
    \multirow{3}{*}{Method} & \multirow{3}{*}{Category} & \multicolumn{2}{c}{Question Types} & \multicolumn{5}{c}{Answer Types} &
    \multicolumn{2}{c}{Grades} &
    \multirow{3}{*}{Avg} \\
    \cmidrule(lr){3-4} \cmidrule(lr){5-9} \cmidrule(lr){10-11} 
    & & MC & FREE & INT & DEC & EXTR & BOOL & OTH & 1-6 & 7-8 & \\
    \midrule
    Random guess & - & 39.81 & 6.71 & 8.37 & 0.26 & 30.80 & 51.22 & 26.67 & 17.55 & 12.27 & 15.29 \\
    Human performance & - & & & \\
    \midrule
    T5$_{\textsc{Large}}$ \citeyearpar{raffel2020exploring} & Training & & & \\
    T5$_{\textsc{3B}}$ \citeyearpar{raffel2020exploring} & Training & & & \\
    UnifiedQA$_{\textsc{Large}}$ \citeyearpar{khashabi2020unifiedqa} & Training & & & \\
    UnifiedQA$_{\textsc{3B}}$ \citeyearpar{khashabi2020unifiedqa} & Training & & & \\
    \midrule
    TAPAS \citeyearpar{herzig2020tapas} & Training & & & \\
    TAPEX \citeyearpar{liu2021tapex} & Training & & & \\
    \midrule    
    Zero-shot GPT-3 \citeyearpar{chen2020big} & Prompting & 66.57 & 53.57 & 55.55 & 45.84 & 78.22 & 55.33 & 53.33 & 63.33 & 48.41 & 56.94 \\
    Zero-shot-CoT GPT-3 \citeyearpar{kojima2022large} & Prompting & 66.92 & 54.36 & 55.82 & 48.67 & 78.82 & 55.67 & 51.43 & 63.62 & 49.59 & 57.61 \\
    Few-shot GPT-3* \citeyearpar{chen2020big} & Prompting & 65.21 & 55.48 & 59.22 & 40.94 & 77.10 & 54.00 & 49.52 & 63.65 & 50.47 & 58.00 \\
    Few-shot-CoT GPT-3* \citeyearpar{wei2022chain} & Prompting & 52.01 & 57.45 & 57.54 & 57.08 & 57.04 & 48.00 & 39.05 & 58.71 & 52.47 & 56.04 \\
    Codex \citeyearpar{chen2021evaluating} & Prompting & & & & \\
    \midrule   
    GPT-3 RLPrompt (ours) & Prompting & & & & \\
    \bottomrule 
    \end{tabular}
 }
 \captionof{table}{Evaluation results of different baselines and our methods on the \data{} dataset. MC: multi-choice questions; FREE: free-text questions; INT: integer answers; DEC: decimal answers; EXTR: extractive text answers; BOOL: boolean text answers; OTH: other text answers.}
 \label{tab:results2}
\end{figure}

==> codes/three_formats.tex <==
\begin{table}[ht!]
\centering
\begin{tabular}{ccc}
\hline
\multicolumn{1}{|c|}{
    \begin{minipage}{0.29\columnwidth}
    \centering
    \fontsize{9.0pt}{\baselineskip}\selectfont
    \vspace{1.0mm}
    \textbf{Image format}
    \vspace{1.0mm}
    \end{minipage}
} 
& \multicolumn{1}{c|}{
    \begin{minipage}{0.36\columnwidth}
    \centering
    \fontsize{9.0pt}{\baselineskip}\selectfont
    \vspace{1.0mm}
    \textbf{Semi-structured format}
    \vspace{1.0mm}
    \end{minipage}
} 
& \multicolumn{1}{c|}{
    \begin{minipage}{0.32\columnwidth}
    \centering
    \fontsize{9.0pt}{\baselineskip}\selectfont
    \vspace{1.0mm}
    \textbf{Structured format}
    \vspace{1.0mm}
    \end{minipage}
} 
\\ 
\hline
\multicolumn{1}{|c|}{
    \begin{minipage}{0.29\columnwidth}
    \centering
    % \vspace{1mm}
    % \hspace{1mm}
    \includegraphics[height=1.4in]{tables/18066.png}
    \end{minipage}
} 
& \multicolumn{1}{l|}{
    \begin{minipage}{0.36\columnwidth}
    \fontsize{7.6pt}{\baselineskip}\selectfont % font size
    \vspace{2mm}
    \textbf{Table title}: Field day schedule \\
    \textbf{Table text}:\\
    Event \(|\)  Begin \(|\)  End\\
    water balloon toss \(|\)  11:30 A.M. \(|\)  11:50 A.M.\\
    obstacle course \(|\)  12:05 P.M. \(|\)  12:25 P.M.\\
    parachute ball toss \(|\)  12:30 P.M. \(|\)  1:30 P.M.\\
    jump rope race \(|\)  1:40 P.M. \(|\)  2:05 P.M.\\
    balloon stomp \(|\)  2:15 P.M. \(|\)  2:35 P.M.\\
    relay race \(|\)  2:50 P.M. \(|\)  3:40 P.M.\\
    hula hoop contest \(|\)  3:55 P.M. \(|\)  4:30 P.M.
    \vspace{1mm}
    \end{minipage}
} 
& \multicolumn{1}{c|}{
    \begin{minipage}{0.32\columnwidth}
    % \hspace{1mm}
    \vspace{2mm}
    \fontsize{7.6pt}{\baselineskip}\selectfont
    \textbf{Table title}: Field day schedule \\
    % \textbf{Table in \textsc{pandas}}: \\
    \includegraphics[height=1.36in]{tables/18066_pandas.png}
    \vspace{1mm}
    \end{minipage}
} 
\\
\hline
\end{tabular}
\caption{Three different formats for the tables in the \data{} dataset.}
\label{tab:three_formats}
\end{table}

==> codes/two_examples.tex <==


% \begin{table*}[t]
% % \small
% % \footnotesize
% % \fontsize{9.0pt}{\baselineskip}\selectfont % font size
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lp{6.0cm}p{12.0cm}}
% \toprule
% \textbf{Task} & \textbf{Question category} & \textbf{Example} \\ 
% \midrule
% \multirow{3}*{\textsc{Task 1}} 
% & Basic math: addition, subtraction, fact based QA etc.
% & \textbf{Original:} If Jimbo is 484 feet away from a beetle and quarter of 827 feet away from a grasshopper, which insect will seem bigger to him??  "Option 1": beetle, "Option 2" :grasshopper \textbf{Answer:} Option 2
% \\
% \bottomrule
% \end{tabular}
% }
% \caption{Example of each task in the \textit{math ability} category of the}
% \label{tab:example}
% % \vspace{-3mm}
% \end{table*}


% \begin{figure}[ht!]
% \vspace{-2mm}
% \centering
% \footnotesize
% \fontsize{8.5pt}{\baselineskip}\selectfont % font size
% \begin{boxedminipage}{0.99\columnwidth}
% \begin{tabular}{ccc}
% \hline
% Name& ID& Gender\\
% \hline
% Steve Jobs& 001& Male\\
% Bill Gates& 002& Female\\
% \hline
% \end{tabular}
% \\
% Question: $\mathtt{question:}$ ${I_i^{ques}}$ \\
% Answer:
% \end{boxedminipage}
% \caption{ABC}
% \vspace{-3mm}
% \label{fig:prompt_encoding}
% \end{figure}



% \begin{figure}[ht!]
% \vspace{-2mm}
% \centering
% \footnotesize
% \fontsize{9.0pt}{\baselineskip}\selectfont % font size
% \begin{boxedminipage}{0.99\columnwidth}
% \vspace{1mm}
% \hspace{10mm}
% \includegraphics[height=1.2in]{figures/fig_acc_diff_cand_num.pdf}
% \\
% Question:  \\
% Options: \\
% Answer:
% \end{boxedminipage}
% \caption{ABC}
% \vspace{-3mm}
% \label{fig:prompt}
% \end{figure}







==> template/datasets.tex <==
\begin{figure}[htb] 
 \centering
% \fontsize{8.5pt}{\baselineskip}\selectfont % font size
% \renewcommand\tabcolsep{3.5pt} % column space
% \renewcommand\arraystretch{0.85} % row space
 \resizebox{1.0\linewidth}{!}{
 \begin{tabular}{lrrrccccccc}
 \toprule
 \multirow{2}*{Dataset} & \multirow{2}*{Size} & \multirow{2}*{AvgQ} & \multirow{2}*{MaxQ} & Tabular & Visual & Generative & Multi-choice & Numeric & Textual & \multirow{2}*{Solution} \\
 & & & & Context & Context & Question & Question & Answer & Answer \\
 \midrule
 MAWPS \citeyearpar{koncel2016mawps} & 2,373 & & & & & \\
 Dolphin18K \citeyearpar{huang2016well} & 18,000 & & & & & \\
 DRAW-1K \citeyearpar{upadhyay2017annotating} & 1,000 & & & & & \\
 Math23K \citeyearpar{wang2017deep} & 23,161 & & & & & \\
 MathQA \citeyearpar{amini2019mathqa} & 37,259 & & & & & \\
 ASDiv-A \citeyearpar{miao2020diverse} & 1218 & & & & & \\
 SVAMP \citeyearpar{patel2021nlp} & 1,000 & & & & & \\
 GSM8K \citeyearpar{cobbe2021training} & 8,792 & & & & & & & & & \cmark\\
 IconQA \citeyearpar{lu2021iconqa} & \textbf{107,439} & 8.4 & 73 & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark \\
 \midrule
 \name{} & \underline{38,431} & 22.1 & 92 & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
% WikiSQL \citep{wang2017deep} & & 26,521 & text & & & \\
% Spider \citep{wang2017deep} & & 1,020 & text & & & \\
% HybridQA \citep{wang2017deep} & & 13,000 & text & & & \\
% TAT-QA \citep{wang2017deep} & & 2,757 & text & & & \\
% FinQA \citep{wang2017deep} & & 2,776 & text & & & \\
% DART \citep{wang2017deep} & & 5,623 & text & & & \\
% LogicNLG \citep{wang2017deep} & & 7,392 & text & & & \\
% ToTTo \citep{wang2017deep} & & 83,141 & text & & & \\
% NumericNLG \citep{wang2017deep} & & 1,300 & text & & & \\
% HiTab \citep{wang2017deep} & & 3,597 & text & & & \\
% \midrule
 \bottomrule
 \end{tabular}
 }
 \captionof{table}{A comparison of existing math word problem datasets. Size: number of problems; MaxQ: maximum number of question words; AvgQ: average number of question words.}
 \label{tab:datasets1}
\end{figure}






\begin{figure}[htb] 
 \centering
 \resizebox{1.0\linewidth}{!}{
\begin{tabular}{lrrrrrcccc}
\toprule
 & \multicolumn{1}{c}{\# Size} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# Avg\\PLen\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# P\\Vocab\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# Diff\\Ans\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\# Max\\ALen\end{tabular}} & Context & \begin{tabular}[c]{@{}c@{}}Question \\types\end{tabular} & \begin{tabular}[c]{@{}c@{}}Answer \\types\end{tabular} & \begin{tabular}[c]{@{}c@{}}Solution\\types\end{tabular} \\
 \midrule
Dolphin18K (2016) & 831 & 17.7 & 601 & 223 & 1 & / & free-text & integer, decimal & formula \\
DRAW-1K (2017) & 1,000 & 32.2 & 2,726 & 465 & 1 & / & free-text & integer, decimal & formula \\
Math23K (2017) & 23,162 & 28.0 & 14,812 & 3,782 & 1 & / & free-text & integer, decimal & formula \\
MathQA (2019) & 37,297 & 34.8 & 12,636 & 6,386 & 1 & / & MC & integer, decimal & formula \\
ASDiv (2020) & 2,305 & 30.7 & 5,304 & 533 & 6 & / & free-text & text, integer, decimal & formula \\
SVAMP (2021) & 1,000 & 31.8 & 840 & 272 & 1 & / & free-text & integer & formula \\
GSM8K (2021) & 8,792 & 45.3 & 15,918 & 983 & 1 & / & free-text & integer & text \\
IconQA (2021) & 107,439 & 8.4 & 2,095 & 1,023 & 8 & diagram & free-text, MC & text, integer & / \\
\midrule
Tab MathQA & \underline{38,431} & \textbf{50.8} & \textbf{22,807} & \underline{6,153} & \textbf{27} & table text/diagram & free-text, MC & text, integer, decimal & text \\
\bottomrule
\end{tabular}
 }
 \captionof{table}{A comparison of existing math word problem datasets. Size: number of problems; MaxQ: maximum number of question words; AvgQ: average number of question words.}
 \label{tab:datasets2}
\end{figure}

\begin{figure}[htb] 
 \centering
 \resizebox{1.0\linewidth}{!}{
\begin{tabular}{lrrrrc|cc|cc|ccc|c} 
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{\#Size} & \multirow{2}{*}{\#AvgP} & \multirow{2}{*}{\#Vocab} & \multirow{2}{*}{\#Ans} & \multirow{2}{*}{\#MaxA} & \multicolumn{2}{c|}{\vcell{Context Type}} & \multicolumn{2}{c|}{\vcell{Question Type}} & \multicolumn{3}{c|}{\vcell{Answer Type}} & \multirow{2}{*}{Solutions} \\[-\rowheight]
 & & & & & & \multicolumn{2}{c|}{\printcellmiddle} & \multicolumn{2}{c|}{\printcellmiddle} & \multicolumn{3}{c|}{\printcellmiddle} & \\ 
\cline{7-13}
 & & & & & & Table & Diagram & Free-text & MC & Text & Integer & Decimal & \\ 
\midrule
Dolphin18K \citeyearpar{huang2016well} & 831 & 17.7 & 601 & 223 & 1 & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & formula \\
DRAW-1K \citeyearpar{upadhyay2017annotating} & 1,000 & 32.2 & 2,726 & 465 & 1 & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & formula \\
Math23K \citeyearpar{wang2017deep} & 23,162 & 28.0 & 14,812 & 3,782 & 1 & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & formula \\
MathQA \citeyearpar{amini2019mathqa} & 37,297 & 34.8 & 12,636 & \textbf{6,386} & 1 & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark & formula \\
ASDiv-A \citeyearpar{miao2020diverse} & 2,305 & 30.7 & 5,304 & 533 & 6 & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark & \cmark & formula \\
SVAMP \citeyearpar{patel2021nlp} & 1,000 & 31.8 & 840 & 272 & 1 & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & formula \\
GSM8K \citeyearpar{cobbe2021training} & 8,792 & 45.3 & 15,918 & 983 & 1 & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & text \\
IconQA \citeyearpar{lu2021iconqa} & \textbf{107,439} & 8.4 & 2,095 & 1,023 & 8 & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \xmark \\ 
\midrule
\name{} & \underline{38,431} & \textbf{50.8} & \textbf{22,807} & \underline{6,153} & \textbf{27} & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & text \\

\bottomrule
\end{tabular}
 }
 \captionof{table}{A comparison of existing math word problem datasets. Size: number of problems; MaxQ: maximum number of question words; AvgQ: average number of question words.}
 \label{tab:datasets3}
\end{figure}


\begin{figure}[htb] 
 \centering
 \resizebox{1.0\linewidth}{!}{
 
\begin{tabular}{lrrrrccccccccc} 
\toprule
\multirow{3}{*}{Dataset} & \multirow{3}{*}{\#Size} & \multirow{2}{*}{\#Avg} & \multirow{2}{*}{\#Prob} & \multirow{2}{*}{\#Diff} & \multirow{2}{*}{\#Max} & \multicolumn{2}{c}{Context Types} & \multicolumn{2}{c}{Question Types} & \multicolumn{3}{c}{Answer Types}	& \multirow{2}{*}{Solution} \\
\cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-13} 
& & PLen & Vocab & Ans & ALen & Table & Diagram & Free-text & MC & Text & Integer & Decimal & Types \\
\midrule
Dolphin18K \citeyearpar{huang2016well} & 831 & 17.7 & 601 & 223 & 1 & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & formula \\
DRAW-1K \citeyearpar{upadhyay2017annotating} & 1,000 & 32.2 & 2,726 & 465 & 1 & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & formula \\
Math23K \citeyearpar{wang2017deep} & 23,162 & 28.0 & 14,812 & 3,782 & 1 & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & formula \\
MathQA \citeyearpar{amini2019mathqa} & 37,297 & 34.8 & 12,636 & \textbf{6,386} & 1 & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark & formula \\
ASDiv-A \citeyearpar{miao2020diverse} & 2,305 & 30.7 & 5,304 & 533 & 6 & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark & \cmark & formula \\
SVAMP \citeyearpar{patel2021nlp} & 1,000 & 31.8 & 840 & 272 & 1 & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & formula \\
GSM8K \citeyearpar{cobbe2021training} & 8,792 & 45.3 & 15,918 & 983 & 1 & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & text \\
IconQA \citeyearpar{lu2021iconqa} & \textbf{107,439} & 8.4 & 2,095 & 1,023 & 8 & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \xmark \\ 
\midrule
\name{} & \underline{38,431} & \textbf{50.8} & \textbf{22,807} & \underline{6,153} & \textbf{27} & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & text \\

\bottomrule
\end{tabular}
 }
 \captionof{table}{A comparison of existing math word problem datasets. Size: number of problems; MaxQ: maximum number of question words; AvgQ: average number of question words.}
 \label{tab:datasets4}
\end{figure}



\begin{figure}[htb] 
 \centering
 \renewcommand\tabcolsep{4.1pt} % column space
%  \renewcommand\arraystretch{0.85} % row space
 \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{p{2.8cm}rrrrccccccccc} 
    \toprule
    \multirow{3}{*}{Dataset} & \multirow{3}{*}{\#Size} & \multirow{2}{*}{\#Avg} & \multirow{2}{*}{\#Prob} & \multirow{2}{*}{\#Diff} & \multirow{2}{*}{\#Max} & \multicolumn{2}{c}{Context Types} & \multicolumn{2}{c}{Question Types} & \multicolumn{3}{c}{Answer Types} & \multirow{2}{*}{Solution} \\
    \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-13} 
    & & PLen & Vocab & Ans & ALen & Table & Diagram & Free-text & MC & Text & Integer & Decimal & Types \\
    \midrule
    Dolphin18K \citeyearpar{huang2016well} & 831 & 17.7 & 601 & 223 & 1 & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & formula \\
    DRAW-1K \citeyearpar{upadhyay2017annotating} & 1,000 & 32.2 & 2,726 & 465 & 1 & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & formula \\
    Math23K \citeyearpar{wang2017deep} & 23,162 & 28.0 & 14,812 & 3,782 & 1 & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & formula \\
    MathQA \citeyearpar{amini2019mathqa} & 37,297 & 34.8 & 12,636 & \textbf{6,386} & 1 & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark & formula \\
    ASDiv-A \citeyearpar{miao2020diverse} & 2,305 & 30.7 & 5,304 & 533 & 6 & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark & \cmark & formula \\
    SVAMP \citeyearpar{patel2021nlp} & 1,000 & 31.8 & 840 & 272 & 1 & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & formula \\
    GSM8K \citeyearpar{cobbe2021training} & 8,792 & 45.3 & 15,918 & 983 & 1 & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & text \\
    IconQA \citeyearpar{lu2021iconqa} & \textbf{107,439} & 8.4 & 2,095 & 1,023 & 8 & \xmark & \cmark & \cmark & \cmark & \cmark & \cmark & \xmark & \xmark \\ 
    \midrule
    SQA \citeyearpar{lu2021iconqa} & & & & & & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\ 
    WTQ \citeyearpar{lu2021iconqa} & & & & & & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\ 
    WikiSQL \citeyearpar{lu2021iconqa} & & & & & & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\ 
    TabFact \citeyearpar{lu2021iconqa} & & & & & & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\ 
    \midrule
    \name{} & \underline{38,431} & \textbf{50.8} & \textbf{22,807} & \underline{6,153} & \textbf{27} & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & text \\
    \bottomrule
    \end{tabular}
 }
 \captionof{table}{A comparison of existing math word problem datasets. \#Size: number of problems; \#AvgPLen: average number of problems; \#ProbVocab: number of problem vocabularies; \#DiffAns: number of different answers; \#MaxPLen: maximum number of answer words.}
 \label{tab:datasets5}
\end{figure}

\begin{figure}[htb] 
 \centering
 \renewcommand\tabcolsep{4.1pt} % column space
% \renewcommand\arraystretch{0.85} % row space
 \resizebox{1.0\linewidth}{!}{
 \begin{tabular}{p{2.8cm}rrrcccccccccc} 
 \toprule
 \multirow{3}{*}{Dataset} & \multirow{3}{*}{Size} & \multirow{3}{*}{\#Table} & \multirow{3}{*}{\#Ques} & \multirow{2}{*}{Need} & \multirow{2}{*}{Need} & \multicolumn{2}{c}{Table Type} & \multicolumn{2}{c}{Question Type} & \multicolumn{3}{c}{Answer Type} & \multirow{2}{*}{Solution} \\
 \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-13} 
 & & & & Math? & Table? & Domain & Format & Free-text & MC & Text & Integer & Decimal & Type \\
 \midrule
Dolphin18K (2016) & 831 & \xmark~~~ & 831 & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & formula \\
DRAW-1K (2017) & 1,000 & \xmark~~~ & 995 & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & formula \\
Math23K (2017) & 23,162 & \xmark~~~ & 23,148 & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark & formula \\
MathQA (2019) & 37,297 & \xmark~~~ & \textbf{36,297} & \cmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark & formula \\
ASDiv (2020) & 2,305 & \xmark~~~ & 2,304 & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark & \cmark & \cmark & formula \\
SVAMP (2021) & 1,000 & \xmark~~~ & 1,000 & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & formula \\
GSM8K (2021) & 8,792 & \xmark~~~ & 8,792 & \cmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark & text \\
IconQA (2021) & \textbf{107,439} & \xmark~~~ & 8,594 & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \cmark & \cmark & \xmark & \xmark \\
\midrule
FinQA (2021) & 8,281 & 2,766 & 8,118 & \cmark & 76.6\% & finance & text & \cmark & \xmark & \xmark & \cmark & \cmark & program \\
TAT-QA (2021) & 16,552 & 2,747 & 15,863 & 22.4\% & \cmark & finance & text & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark \\
MultiHiertt (2022) & 10,440 & 9,843 & 10,440 & \cmark & 89.8\% & finance & text & \cmark & \xmark & \xmark & \cmark & \cmark & \xmark \\
\midrule
\textbf{\name{}} & \textbf{38,431} & \textbf{37,644} & 28,876 & \cmark & \cmark & \textbf{open} & \textbf{text/image} & \cmark & \cmark & \cmark & \cmark & \cmark & \textbf{text}\\
\bottomrule
 \end{tabular}
 }
 \captionof{table}{A comparison of existing math word problem datasets. \#Size: number of problems; \#AvgPLen: average number of problems; \#ProbVocab: number of problem vocabularies; \#DiffAns: number of different answers; \#MaxPLen: maximum number of answer words.}
 \label{tab:datasets6}
\end{figure}
